FuSS: Fusing Superpixels for Improved Segmentation Consistency

In this work, we propose two different approaches to improve the semantic consistency of Open Set Semantic Segmentation. First, we propose a method called OpenGMM that extends the OpenPCS framework using a Gaussian Mixture of Models to model the distribution of pixels for each class in a multimodal manner. The second approach is a post-processing which uses superpixels to enforce highly homogeneous regions to behave equally, rectifying erroneous classified pixels within these regions, we also proposed a novel superpixel method called FuSS. All tests were performed on ISPRS Vaihingen and Potsdam datasets, and both methods were capable to improve quantitative and qualitative results for both datasets. Besides that, the post-process with FuSS achieved state-of-the-art results for both datasets. The official implementation is available at: \url{https://github.com/iannunes/FuSS}.

==> files/table_ablation_score.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
    \centering
    % \resizebox{\textwidth}{!}{%
        \begin{tabular}{cccccccc}
            \hline
            \multicolumn{5}{c}{\textbf{UUCs}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Average}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Prediction}}} & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Value Used}}} \\ \cline{1-5}
            \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{3}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{l}{} \\ \hline
            %.904 & \textbf{.959} & .733 & .880 & .881 & $.8714 \pm .083$ & True & All \\
            %.904 & \textbf{.959} & .733 & .880 & .881 & $.8714 \pm .083$ & False & All \\
            %.903 & .958 & \textbf{.737} & \textbf{.881} & \textbf{.897} & $.8751 \pm .083$ & All & Mean \\
            %\textbf{.906} & \textbf{.959} & .730 & .880 & .864 & $.8676 \pm .085$ & All & Median \\
            .903 & .958 & \textbf{.737} & \textbf{.881} & \textbf{.897} & $\mathbf{.875 \pm .083}$ & True & Mean \\
            \textbf{.906} & \textbf{.959} & .730 & .880 & .865 & $.868 \pm .085$ & True & Median \\
            .903 & .958 & \textbf{.737} & \textbf{.881} & \textbf{.897} & $\mathbf{.875 \pm .083}$ & False & Mean \\
            \textbf{.906} & \textbf{.959} & .730 & .880 & .865 & $.868 \pm .085$ & False & Median
        \end{tabular}%
    % }
    \caption{The table shows the AUROC results for all the 70 different superpixel configurations executed for the ablation aggregated how they were applied to the Score/Reconstruction Error generated by de OSS methods. UUCs are presented as the average AUROC; if the superpixel segmentation was applied to all prediction output and to the score/reconstruction error the column ``Prediction'' is set to True, if it is only used for the score/reconstruction error is set to False; the last column shows which value is used to represent the entire superpixel when applied to all pixels of the segmented score/reconstruction error. The numbered UUC columns stands for: 0 - impervious surfaces; 1 - buildings; 2 - low vegetation; 3 - high vegetation; 4 - car.}
    \label{tab:ablation_scores}
\end{table*}
